Planar Reflection-Aware Neural Radiance Fields

Neural Radiance Fields (NeRF) have demonstrated exceptional capabilities in reconstructing complex scenes with high fidelity. However, NeRF's view dependency can only handle low-frequency reflections. It falls short when handling complex planar reflections, often interpreting them as erroneous scene geometries and leading to duplicated and inaccurate scene representations. To address this challenge, we introduce a reflection-aware NeRF that jointly models planar reflectors, such as windows, and explicitly casts reflected rays to capture the source of the high-frequency reflections. We query a single radiance field to render the primary color and the source of the reflection. We propose a sparse edge regularization to help utilize the true sources of reflections for rendering planar reflections rather than creating a duplicate along the primary ray at the same depth. As a result, we obtain accurate scene geometry. Rendering along the primary ray results in a clean, reflection-free view, while explicitly rendering along the reflected ray allows us to reconstruct highly detailed reflections. Our extensive quantitative and qualitative evaluations of real-world datasets demonstrate our method's enhanced performance in accurately handling reflections.

==> 5_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

We have presented a new method for accurately modeling planar reflections for scene reconstruction and novel view synthesis.
Our reflection-aware NeRF jointly models the planar surfaces and explicitly casts reflected rays to capture the \emph{source} of the high-frequency reflections. 
Our core idea is to maintain a \emph{single} geometry and appearance instance. 
If a real object is present along the reflected ray, unlike NeRF, our method does not create a false duplicate along the primary ray at the same depth to explain the reflection. 
Instead, it uses the reflected ray to explain the reflection, ensuring the primary view is clean and accurate.
We validate the effectiveness of our method on on a challenging real-world 360-degree dataset, demonstrating its superior performance in comparison to current state-of-the-art methods.

==> figures/edge_loss_calculation.tex <==
\begin{figure}[t]
\centering%
\parbox[t]{1\linewidth}{\centering%
\includegraphics[width=1\linewidth]{fig/edge_loss_calculation_v2.pdf}}
\caption{\textbf{False geometry.}
The network tends to create false geometry along the primary ray, mirroring the actual object's position as observed along the reflected ray to explain the reflections. 
% To mitigate this issue of duplication, we constrain the gradients of both primary and reflected colors.
% Our sparse edge regularization is defined by minimizing the element-wise multiplication between these two sets of gradients.
% This regularization is only applied to constrain the primary colors.
% \changil{It's not clear what images want to say. What do the two colors mean? What do the insets represent? Explain the visuals in the caption. You don't have to explain the sparse edge regularization in the caption; just mention it will handle what's shown in this image. Also this figure is too big to the amount of information it would convey. Show the renderings of the primary and reflected rays at least. I think you had some really cool visualizations of false geometry, gradients, etc. that you used for our discussions meetings. Maybe you can reuse some?}
\chen{Seems duplicated. We show similar results in the motivation figure.}
}
\label{fig:edge_loss_calculation}
\end{figure}

==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}


==> setup/package.tex <==
% Fix "undefined control sequence \Everyshipout".
% \usepackage{everyshi}

% Figures
% \usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}                                         % Useful for wide tables or figures.
\usepackage{wrapfig}

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}
\usepackage{animate} %% convert frames to video

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{makecell}

\usepackage{paralist}
\usepackage{enumitem}
\setlist[enumerate]{itemsep=0mm}

% Math
\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
\usepackage{graphicx}                  % another package that works for figures
\usepackage{times}
\usepackage{mathptmx}
\usepackage{mathtools}
\usepackage{amssymb,amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% Fonts
\usepackage{units}
\usepackage{color}
\usepackage{xcolor}

% Comments
\usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
% \usepackage{xspace}
% \usepackage[table]{xcolor}
% \usepackage{setspace}
% \usepackage{grfext}
% \PrependGraphicsExtensions*{.jpg,.png,.PNG}

\usepackage{gensymb}
% \usepackage{emoji}

% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}

